Search for dark matter in association with a Higgs boson decaying to $b$-quarks in $pp$ collisions at $\sqrt{s} = 13$ TeV with the ATLAS detector

A search for dark matter pair production in association with a Higgs boson decaying to a pair of bottom quarks is presented, using 3.2 $fb^{-1}$ of $pp$ collisions at a centre-of-mass energy of 13 TeV collected by the ATLAS detector at the LHC. The decay of the Higgs boson is reconstructed as a high-momentum $b\bar{b}$ system with either a pair of small-radius jets, or a single large-radius jet with substructure. The observed data are found to be consistent with the expected backgrounds. Results are interpreted using a simplified model with a $Z'$ gauge boson mediating the interaction between dark matter and the Standard Model as well as a two-Higgs-doublet model containing an additional $Z'$ boson which decays to a Standard Model Higgs boson and a new pseudoscalar Higgs boson, the latter decaying into a pair of dark matter particles.

==> jetetmisssymbols.tex <==
%%% For boosted stuff
\newcommand{\mjet}      {\ensuremath{m^{\rm jet}}\xspace}
\newcommand{\pti}       {\ensuremath{p_{{\rm T}i}}\xspace}
\newcommand{\fcut}      {\ensuremath{f_{\rm cut}}\xspace}
\newcommand{\Rsub}      {\ensuremath{R_{\rm sub}}\xspace}
\newcommand{\largeR}    {large-\ensuremath{R}\xspace}
\newcommand{\LargeR}    {Large-\ensuremath{R}\xspace}
\newcommand{\smallR}    {small-\ensuremath{R}\xspace}
\newcommand{\SmallR}    {Small-\ensuremath{R}\xspace}
\newcommand{\hhbbbb}    {\ensuremath{hh\rightarrow4b}\xspace}


%%% Energy
\newcommand{\fourfgev}    {\ensuremath{450~\mathrm{GeV}}\xspace}
\newcommand{\ninehgev}    {\ensuremath{900~\mathrm{GeV}}\xspace}
\newcommand{\seventev}    {\ensuremath{7~\mathrm{TeV}}\xspace}
\newcommand{\eighttev}    {\ensuremath{8~\mathrm{TeV}}\xspace}
\newcommand{\fourteentev} {\ensuremath{14~\mathrm{TeV}}\xspace}
\newcommand{\sqsTev}      {\ensuremath{1.96~\mathrm{TeV}}\xspace}
\newcommand{\threehtev}   {\ensuremath{3.5~\mathrm{TeV}}\xspace}
\newcommand{\sqsnineh}    {\ensuremath{\sqrt{s} = \ninehgev}\xspace}
\newcommand{\sqsseven}    {\ensuremath{\sqrt{s} = \seventev}\xspace}
\newcommand{\sqseight}    {\ensuremath{\sqrt{s} = \eighttev}\xspace}
\newcommand{\sqsfourt}    {\ensuremath{\sqrt{s} = \fourteentev}\xspace}

%%% Event generator stuff
%\newcommand{\Herwig}    {\textsc{HERWIG}\xspace}
%\newcommand{\herwigpp}  {\textsc{HERWIG}++\xspace}
%\newcommand{\Herwigpp}  {\herwigpp}
%\newcommand{\geant}     {G\textsc{eant}4\xspace}
\newcommand{\geant}     {\textsc{Geant4}\xspace}
\newcommand{\jimmy}     {\textsc{JIMMY}\xspace}
\newcommand{\Alpgen}    {\textsc{ALPGEN}\xspace}
\newcommand{\Mcatnlo}   {\textsc{MC@NLO}\xspace}
\newcommand{\Acermc}    {\textsc{AcerMC}\xspace}
\newcommand{\Sherpa}    {\textsc{SHERPA}\xspace}
\newcommand{\Comphep}   {\textsc{CompHep}\xspace}
\newcommand{\Madgraph}  {\textsc{MadGraph}\xspace}
\newcommand{\Pythia}    {\textsc{PYTHIA}\xspace}
\newcommand{\pythiaeight}   {\textsc{Pythia8}\xspace}
\newcommand{\Powheg}    {\textsc{POWHEG}\xspace}
\newcommand{\PowhegBox} {\Powheg-BOX\xspace}
\newcommand{\PowPythia} {\textsc{POWHEG}+\Pythia}
\newcommand{\HJimmy}    {\textsc{HERWIG}+\jimmy}
\newcommand{\Perugia}   {\textsc{PERUGIA}\xspace}
\newcommand{\PythiaP}   {\Pythia (\Perugia 2010)\xspace}
\newcommand{\ntilde}    {{\~ n}}
\newcommand{\LO}        {\ensuremath{\mathrm{LO}}\xspace}
\newcommand{\NLO}       {\ensuremath{\mathrm{NLO}}\xspace}
\newcommand{\NNLO}      {\ensuremath{\mathrm{N}}\NLO\xspace}
\newcommand{\nLO}       {\nbar \LO\xspace}
\newcommand{\nNLO}      {\nbar \NLO\xspace}
\newcommand{\nnNLO}     {\nbar \nbar \NLO\xspace}
\newcommand{\nnLO}      {\nbar \nbar \LO\xspace}
\newcommand{\nNNLO}     {\nbar \NNLO\xspace}
\newcommand{\muF}       {\ensuremath{\mu_\textsc{f}}\xspace}
\newcommand{\muR}       {\ensuremath{\mu_\textsc{r}}\xspace}
\newcommand{\LS}        {\ensuremath{\mathrm{LS}}\xspace}
\newcommand{\nlojet}    {\textsc{NLOJet}\texttt{++}\xspace}

% Processes
\newcommand{\W}         {\Wboson\xspace}
\newcommand{\Z}         {\Zboson\xspace}
\newcommand{\enu}       {\ensuremath{e\nu}\xspace}  
\newcommand{\Zmumu}     {\ensuremath{Z\ra\mumu}\xspace}
\newcommand{\Wlnu}      {\ensuremath{W\ra \lnu}\xspace}
\newcommand{\Wenu}      {\ensuremath{W\ra \enu}\xspace}
\newcommand{\munu}      {\ensuremath{\mu\nu}\xspace}
\newcommand{\Wmunu}     {\ensuremath{W\ra\munu}\xspace}
\newcommand{\Wjets}     {\Wboson+jets\xspace}
\newcommand{\Zjets}     {\Zboson+jets\xspace}

\newcommand{\inwork}{{\bf This figure is still WORK IN PROGRESS.}}

\newcommand{\antikt}{anti-$k_{t}$}
\newcommand{\Antikt}{Anti-$k_{t}$}
\newcommand{\asym}{\ensuremath{\mathcal{A}}}
\newcommand{\Fastjet} {{\sc FastJet}\xspace}

%%% Luminosity
\newcommand{\invpb}     {~\ensuremath{{\rm pb}^{-1}}\xspace}
\newcommand{\invnb}     {~\ensuremath{{\rm nb}^{-1}}\xspace}
\newcommand{\invfb}     {~\ensuremath{{\rm fb}^{-1}}\xspace}
\newcommand{\invmub}    {~\ensuremath{\mu{\rm b}^{-1}}\xspace}
\newcommand{\cmSqSec}   {cm\ensuremath{^{-2}}s\ensuremath{^{-1}}\xspace}
\newcommand{\lumi}      {\ensuremath{\mathcal L}\xspace}
\newcommand{\calL}      {\lumi}
\newcommand{\dldz}      {\ensuremath{d\lumi/dz}\xspace}
\newcommand{\lofz}      {\ensuremath{{\mathcal L}(z)}\xspace}
\newcommand{\sigyofz}   {\ensuremath{\sigma_y(z)}\xspace}
\newcommand{\Lsp}       {\ensuremath{{\mathcal L}_{sp}}\xspace}
\newcommand{\StoB}      {\ensuremath{S/B}\xspace}
\newcommand{\pileup}    {pile-up\xspace}
\newcommand{\Pileup}    {Pile-up\xspace}

 
             
% pileup subtraction related
\newcommand{\ghostpt}     {\ensuremath{g_{t}}\xspace}
\newcommand{\ghostptavg}  {\ensuremath{\langle\ghostpt\rangle}\xspace}
\newcommand{\ghostfm}     {\ensuremath{g_{\mu}}\xspace}
\newcommand{\ghostfmi}    {\ensuremath{g_{\mu,i}}\xspace}
\newcommand{\ghostdensity}{\ensuremath{\nu_{g}}\xspace}
\newcommand{\ghostrho}    {\ensuremath{\ghostdensity\ghostptavg}\xspace}
\newcommand{\Aghost}      {\ensuremath{A_{g}}\xspace}
\newcommand{\Amu}         {\ensuremath{A_{\mu}}}
\newcommand{\Amui}        {\ensuremath{A_{\mu, i}}}
\newcommand{\jetarea}     {\ensuremath{A^{\mathrm{jet}}}\xspace}
\newcommand{\jetareafm}   {\ensuremath{A^{\mathrm{jet}}_{\mu}}\xspace}
\newcommand{\jetareai}    {\ensuremath{\jetarea_{i}}\xspace}
\newcommand{\rkt}         {\ensuremath{R_{\kt}}\xspace}

%
\newcommand{\JES}   {{\rm JES}}
\newcommand{\JMS}   {{\rm JMS}}
\newcommand{\EMJES} {{\rm EM+JES}}
\newcommand{\GCWJES}{{\rm GCW+JES}}
\newcommand{\LCWJES}{{\rm LCW+JES}}
\newcommand{\EM}    {{\rm EM}}
\newcommand{\GCW}   {{\rm GCW}}
\newcommand{\LCW}   {{\rm LCW}}
%
\newcommand{\GSL}   {{\rm GSL}}
\newcommand{\GS}    {{\rm GS}}

\newcommand{\MTF}   {{\rm MTF}}
\newcommand{\MPF}   {{\rm MPF}}
\newcommand{\Etmiss}   {\ensuremath{{E}_{\mathrm{T}}^{\mathrm{miss}}}}
\newcommand{\vecEtmiss}{\ensuremath{\vec{E}_{\mathrm{T}}^{\mathrm{miss}}}}

\newcommand{\EoverP}    {\ensuremath{E/p}}
\newcommand{\Etrue}     {\ensuremath{E^{\rm truth}}}
\newcommand{\Etruth}    {\ensuremath{E^{\rm truth}}}
\newcommand{\Ecalo}     {\ensuremath{E^{\rm jet}}}
\newcommand{\EcaloEM}   {\ensuremath{E^{\rm jet}_\EM}}
\newcommand{\Response}  {\ensuremath{\mathcal{R}}} 
\newcommand{\Rcalo}     {\ensuremath{\Response^{\rm jet}}} 
\newcommand{\RcaloM}    {\ensuremath{\Response^{\rm jet}_{M}}} 
\newcommand{\RcaloEM}   {\ensuremath{\Rcalo_\EM}}
\newcommand{\RMPF}      {\ensuremath{\Response_\MPF}}
\newcommand{\EcaloCALIB}{\ensuremath{E^{\rm jet}}}
\newcommand{\RcaloCALIB}{\ensuremath{\mathcal{R}^{\rm jet}}}

\newcommand{\EcaloEMJES} {\ensuremath{E^{\rm jet}_\EMJES}}
\newcommand{\RcaloEMJES} {\ensuremath{\mathcal{R}^{\rm jet}_\EMJES}}
\newcommand{\EcaloGCWJES}{\ensuremath{E^{\rm jet}_\GCWJES}}
\newcommand{\RcaloGCWJES}{\ensuremath{\mathcal{R}^{\rm jet}_\GCWJES}}
\newcommand{\EcaloLCWJES}{\ensuremath{E^{\rm jet}_\LCWJES}}
\newcommand{\RcaloLCWJES}{\ensuremath{\mathcal{R}^{\rm jet}^\LCWJES}}
\newcommand{\Rtrack}     {\ensuremath{\mathcal{R}^{\rm track  \; jet}}}

\newcommand{\rtrk}             {\ensuremath{r_{\rm trk}}\xspace}
\newcommand{\rtrksubjet}       {\ensuremath{r^{\rm subjet}_{\rm trk}}\xspace}
\newcommand{\Rtrk}             {\ensuremath{R_{\rm trk}}\xspace}
\newcommand{\rtrackjet}        {\ensuremath{r^{\rm calo / track \; jet}}}
\newcommand{\rtrackjetiso}     {\ensuremath{\rtrackjet_{\rm iso}}}
\newcommand{\rtrackjetnoniso}  {\ensuremath{\rtrackjet_{\rm non-iso}}}
\newcommand{\rtrackjetisoratio}{\ensuremath{\rtrackjet_{\rm non-iso/iso}}}

\newcommand{\Rmin}       {\ensuremath{R_{\rm min}}}
\newcommand{\DeltaR}     {\ensuremath{\Delta R}}
\newcommand{\Dy}         {\ensuremath{\Delta y}\xspace}
\newcommand{\Deta}       {\ensuremath{\Delta\eta}\xspace}
\newcommand{\Dphi}       {\ensuremath{\Delta\phi}\xspace}
\newcommand{\DetaDphi}   {\ensuremath{\sqrt{(\Deta)^{2} + (\Dphi)^{2}}}\xspace}
\newcommand{\DyDphi}     {\ensuremath{\sqrt{(\Dy)^{2} + (\Dphi)^{2}}}\xspace}
\newcommand{\DeltaRdef}  {\ensuremath{\DeltaR = \DetaDphi}\xspace}
\newcommand{\DeltaRydef} {\ensuremath{\DeltaR = \DyDphi}\xspace}
\newcommand{\DeltaRtrk}  {\ensuremath{\Delta R({\rm trk}_1,{\rm trk}_2)}}

\newcommand{\JVF}       {\ensuremath{JVF}\xspace}

\newcommand{\etaDet}{\ensuremath{\eta_{\rm det}}}
%
\newcommand{\etatrk}{\ensuremath{\eta^{\rm track}}}

\newcommand{\etaRange}[2]{\ensuremath{{#1}\leq|\eta|<{#2}}}
\newcommand{\AetaRange}[1]{\ensuremath{|\eta|<{#1}}}

\newcommand{\gammajet}{\ensuremath{\gamma}\mbox{-}{\rm jet}}
\newcommand{\deltaphijetgamma}{\ensuremath{\Delta \phi_{{\rm jet}\mbox{-}\ensuremath{\gamma}}}}
\newcommand{\Zbb}     {\ensuremath{Z\ra\bbbar}\xspace}
\newcommand{\tWb}     {\ensuremath{t \ra Wb}\xspace}
\newcommand{\Wqqbar}  {\ensuremath{W \ra \qqbar}\xspace}

\def\ltap{\raisebox{-.4ex}{\rlap{$\sim$}} \raisebox{.4ex}{$<$}}
\def\gtap{\raisebox{-.4ex}{\rlap{$\sim$}} \raisebox{.4ex}{$>$}}


\newcommand{\insitu}   {{\textit{in situ}}\xspace}
\newcommand{\Insitu}   {{\textit{In situ}}\xspace}
\newcommand{\pp}       {\ensuremath{pp}\xspace}

\newcommand{\etjet}    {\ensuremath{\et^{\mathrm{jet}}}\xspace}
\newcommand{\ptavg}    {\ensuremath{\pt^\mathrm{avg}}\xspace}
\newcommand{\ptjet}    {\ensuremath{\pt^\mathrm{jet}}\xspace}
\newcommand{\ptjeti}   {\ensuremath{p_{\mathrm{T}, i}^\mathrm{jet}}\xspace}
\newcommand{\ptRecoil} {\ensuremath{\pt^\mathrm{Recoil}}}
\newcommand{\ptLeading}{\ensuremath{\pt^\mathrm{Leading}}}
\newcommand{\ptjetEM}  {\ensuremath{p_{\rm T, \EM}^\mathrm{jet}}}
\newcommand{\pthat}    {\ensuremath{\hat{p}_{\rm T}}}
\newcommand{\ptprobe}  {\ensuremath{\pt^{\mathrm{probe}}}}
\newcommand{\ptref}    {\ensuremath{\pt^{\mathrm{ref}}}}
\newcommand{\Zpt}      {\ensuremath{\pt^{Z}}\xspace}
\newcommand{\Wpt}      {\ensuremath{\pt^{\Wboson}}\xspace}
\newcommand{\toppt}    {\ensuremath{\pt^{\rm t}}\xspace}
%
\newcommand{\ptRange}[2]{\ensuremath{{#1} \leq \ptjet<{#2} \GeV}}
\newcommand{\pttrue}  {\ensuremath{\pt^\mathrm{truth}}}
\newcommand{\pttruth} {\ensuremath{\pt^{\mathrm{truth}}}}
\newcommand{\pttrk}   {\ensuremath{\pt^{\mathrm{track}}}} 
\newcommand{\ptrk}    {\ensuremath{p^{\mathrm{track}}}} 
\newcommand{\pTtrkjet}{\ensuremath{p^{\mathrm{track \; jet}}_{\rm T}}}
\newcommand{\ntrk}    {\ensuremath{n_{\rm track}}} 

\newcommand{\sumPt}       {\ensuremath{\sum \vec{p}_{ \rm T}}}
\newcommand{\sumPtTr}     {\ensuremath{|\sum \vec{p}_{\rm T}^{\rm  track}|}}
\newcommand{\sumPtTrk}    {\ensuremath{\sum\pt^{\rm \ track}}\xspace}
\newcommand{\sumPtTrkSq}  {\ensuremath{\sum(\pt^{\rm \ track})^{2}}\xspace}

\newcommand{\ptf}{\ensuremath{\pt^{\rm f}}}
\newcommand{\ptc}{\ensuremath{\pt^{\rm c}}}
\newcommand{\ptl}{\ensuremath{\pt^{\rm left}}}
\newcommand{\ptr}{\ensuremath{\pt^{\rm right}}}

\newcommand{\rapjet}{\ensuremath{y}}
\newcommand{\etajet}{\ensuremath{\eta}}
\newcommand{\phijet}{\ensuremath{\phi}}

\newcommand{\radlength}{\ensuremath{X_0}}


\newcommand{\topo} {topo-clust\-er}
\newcommand{\Topo} {Topo-clust\-er}
\newcommand{\topos}{topo-clust\-ers}
\newcommand{\Topos}{Topo-clust\-ers}

\newcommand{\central}{$0.3$ \ensuremath{\leq |\eta| < } $0.8$}
\newcommand{\ecap}   {$2.1$ \ensuremath{\leq |\eta| < } $2.8$}
\newcommand{\forward}{$3.6$ \ensuremath{\leq |\eta| < } $4.5$}

\newcommand{\Npv}     {\ensuremath{N_{\rm PV}}\xspace}
\newcommand{\NtrkPV}  {\ensuremath{N^{\rm PV}_{\rm track}}\xspace}
\newcommand{\Nref}    {\ensuremath{\Npv^{\rm ref}}\xspace}
\newcommand{\Navg}    {\ensuremath{\langle \Npv \rangle}\xspace}
\newcommand{\bunchSp} {\ensuremath{\tau_{\rm bunch}}\xspace}
\newcommand{\avgmu}   {\ensuremath{\langle \mu \rangle}\xspace}

\newcommand{\ATLAS}   {ATLAS}
\newcommand{\Lone}    {\texttt{L1}}
\newcommand{\HLT}     {\texttt{HLT}}
\newcommand{\ID}      {\texttt{ID}}
\newcommand{\Pixel}   {\texttt{Pixel}}
\newcommand{\SCT}     {\texttt{SCT}}
\newcommand{\TRT}     {\texttt{TRT}}

\newcommand{\LHC}    {LHC}
\newcommand{\EMB}    {\texttt{EMB}}
\newcommand{\EME}    {\texttt{EME}}
\newcommand{\EMEC}   {\texttt{EMEC}}
\newcommand{\FCAL}   {\texttt{FCAL}}
\newcommand{\Cryo}   {\texttt{Cryo}}
\newcommand{\Gap}    {\texttt{Gap}}
\newcommand{\Scint}  {\texttt{Scint}}
\newcommand{\HEC}    {\texttt{HEC}}
\newcommand{\LAr}    {\texttt{LAr}}
\newcommand{\FCal}   {\texttt{FCal}}
\newcommand{\Tile}   {\texttt{Tile}}
\newcommand{\TileExt}{\texttt{TileExt}}
\newcommand{\TileBar}{\texttt{TileBar}}
\newcommand{\MBTS}   {\texttt{MBTS}}
\newcommand{\Presampler}   {\texttt{Presampler}}

%
\newcommand{\width}   {{\rm width}}

\newcommand{\ftile}{\ensuremath{f_{\Tile 0}}}
\newcommand{\fem}  {\ensuremath{f_{\LAr 3}}}
\newcommand{\fpres}{\ensuremath{f_{\rm PS}}}
\newcommand{\fhec} {\ensuremath{f_{\HEC 0}}}
\newcommand{\ffcal}{\ensuremath{f_{\FCal 1}}}


\newcommand{\btag   }{{\ensuremath{b}\mbox{\rm-tagging}}}
\newcommand{\btagged}{{\ensuremath{b}\mbox{\rm-tagged}}}
\newcommand{\bquark }{{\ensuremath{b}\mbox{\rm-quark}}}
\newcommand{\bquarks}{{\ensuremath{b}\mbox{\rm-quarks}}}
%
\newcommand{\bjet}{{\ensuremath{b}\mbox{-}{\rm jet}}}
\newcommand{\bjets}{{\ensuremath{b}\mbox{\rm-jets}}}

\newcommand{\parentjet }{{\rm parent\, jet}\xspace}
\newcommand{\Parentjet }{{\rm Parent\, jet}\xspace}
\newcommand{\parentjets}{{\rm parent\, jets}\xspace}
\newcommand{\Parentjets}{{\rm Parent\, jets}\xspace}
%


==> journal/Makefile <==
# Makefile for creating an ATLAS paper draft using journal classes

TEXLIVE  = 2013
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
DVIPS    = dvips
DVIPDF   = dvipdf
OPEN     = open

TEXFILES = $(wildcard *.tex)

.PHONY: texlive clean

all: atlas-elsevier atlas-jhep atlas-revtex

texlive:
	for file in $(TEXFILES); do \
	  if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	    echo "Changing texlive value in $$file"; \
	    sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $$file; \
	  else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \
	done

atlas-elsevier: atlas-elsevier.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-jhep: atlas-jhep.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-revtex: atlas-revtex.pdf
	@echo "Made $<"
	# $(OPEN) $<

run_latex: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $< and $(basename $<).pdf"

# Standard LaTeX targets
%.pdf: %.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.dvi: $(BASENAME).tex
	$(LATEX)    $<
	$(LATEX)    $<

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf \
	 *.spl *-revtexNotes.bib *.run.xml *.synctex.gz *~

cleanall: clean
	-rm *.pdf


==> journal/atlas-document-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

%% Title
\AtlasTitle{A simple ATLAS paper draft}
%
% Author - this does not work with revtex
% \author{The ATLAS Collaboration}
%
% Date: if not given, uses current date
% \date{\today}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in final version.
\AtlasVersion{1.0}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{GROUP-2014-XX}

% ATLAS note number. Can be an COM, INT, PUB or CONF note
% \AtlasNote{ATLAS-CONF-2014-XXX}
% \AtlasNote{ATLAS-PUB-2014-XXX}
\AtlasNote{ATLAS-COM-PHYS-2014-XXX}

% Submission journal
\AtlasJournal{Phys.\ Lett.\ B.}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
	This is a bare bones ATLAS document used to demonstrate how to use journal templates.

	This document is typeset using the \DocumentStyle.
}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% Explicit list of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
\AtlasCoverSupportingNote{A supporting note}{http://cds.cern.ch/record/XXXXXX}
\AtlasCoverSupportingNote{Another supporting note}{http://cds.cern.ch/record/YYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
\AtlasCoverCommentsDeadline{DD Month 2014}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
\AtlasCoverAnalysisTeam{Peter Analyser, Susan Editor1, Jenny Editor2, Alphonse Physicien}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
\AtlasCoverEdBoardMember{EdBoard~Chair~(chair), EB~Member~1, EB~Member~2, EB~Member~3}

% Editors egroup
\AtlasCoverEgroupEditors{atlas-GROUP-2014-XX-editors@cern.ch}

% EdBoard egroup
\AtlasCoverEgroupEdBoard{atlas-GROUP-2014-XX-editorial-board@cern.ch}

% CERN preprintnumber
\PreprintIdNumber{CERN-PH-2014-XX}

